Dynamical Friction in Interacting Relativistic Systems

We study dynamical friction in interacting relativistic systems with arbitrary mean free paths and medium constituent masses. Our novel framework recovers the known limits of ideal gas and ideal fluid when the mean free path goes to infinity or zero, respectively, and allows for a smooth interpolation between these limits. We find that in an infinite system the drag force can be expressed as a sum of ideal-gas-like and ideal-fluid-like contributions leading to a finite friction even at subsonic velocities. This simple picture receives corrections in any finite system and the corrections become especially significant for a projectile moving at a velocity $v$ close to the speed of sound $v\approx c_s$. These corrections smoothen the ideal fluid discontinuity around the speed of sound and render the drag force a continuous function of velocity. We show that these corrections can be computed to a good approximation within effective theory of viscous fluid dynamics.

==> freestream.tex <==
% !TEX root = main_file.tex

In this appendix will will cover several technical steps of the calculation that we perform 
in Sec~\ref{subsec:freestream}. First, in order to get the force we are interested 
in the dressed graviton propagator. In our formalism the integral expression from 
this object reads
{\small
\beq
G^{dressed} = \int \frac{d^3p}{(2\pi)^3 } \left(
\frac{\kappa }{-(\omega + i \epsilon)^2 + k^2 }  
\right)^2 I_{\gamma \delta, \mu \nu} I_{\alpha \beta, \rho \sigma}
\frac{\delta \Gamma^i_{\phantom{\alpha} \omega \xi}}{\delta h_{\rho \sigma }}
\frac{p^\mu p^\nu p^\omega p^\xi}{(p^0)^2 T}
\frac{f_0'(p^0/T)}{-i \omega + i \vec k \cdot  \frac{\vec p}{p^0}} u^\gamma u^\delta
u^\rho u^\sigma
\eeq  
}where as usual $p^0 = \sqrt{\vec p^2 + m^2}$.
One can analytically perform the angular integration in the momentum space and project 
onto the four-velocities of the bullet to get an expression of the following form:
\beq\nonumber 
G^{dressed} &= & - \int \frac{dp\  p^3\ f_0'(p^0/T)\ \gamma^2}{240 \pi^2 \ T \ (p^0)^2 \ (k_\perp^2 
	+ k_z^2)^{9/2} (k_\perp^2 +k_z^2 (1 - v^2))^2} \bigg( R(p, p^0; k_\perp, k_z; v) + \\
 &&
 S(p, p^0; k_\perp, k_z; v) \log \frac{k_z p^0 v + 
 	p\sqrt{k_\perp^2 + k_z^2}}{k_z p_0 v -p \sqrt{k_\perp^2 + k_z^2}}
\bigg)
\eeq 
after we have substituted $\omega = k_z v$. 
Functions $R$ and $S$ are polynomial in variables in all their variables. Moreover, $R$
is a perfectly even function of $k^z$ and therefore it does not contribute to the final integral 
over $k_z$. The function $S$ does contribute though, while the contribution to the imaginary part
comes from the jump over the log branch cut. 
Finally, using \eqref{eq:fzintegral}, we find \eqref{eq:free_stream_result}.


